Graph Theoretical Analysis of local ultraluminous infrared galaxies and quasars

We present a methodological framework for studying galaxy evolution by utilizing Graph Theory and network analysis tools. We study the evolutionary processes of local ultraluminous infrared galaxies (ULIRGs) and quasars and the underlying physical processes, such as star formation and active galactic nucleus (AGN) activity, through the application of Graph Theoretical analysis tools. We extract, process and analyse mid-infrared spectra of local (z < 0.4) ULIRGs and quasars between 5-38 microns through internally developed Python routines, in order to generate similarity graphs, with the nodes representing ULIRGs being grouped together based on the similarity of their spectra. Additionally, we extract and compare physical features from the mid-IR spectra, such as the polycyclic aromatic hydrocarbons (PAHs) emission and silicate depth absorption features, as indicators of the presence of star-forming regions and obscuring dust, in order to understand the underlying physical mechanisms of each evolutionary stage of ULIRGs. Our analysis identifies five groups of local ULIRGs based on their mid-IR spectra, which is quite consistent with the well established fork classification diagram by providing a higher level classification. We demonstrate how graph clustering algorithms and network analysis tools can be utilized as unsupervised learning techniques for revealing direct or indirect relations between various galaxy properties and evolutionary stages, which provides an alternative methodology to previous works for classification in galaxy evolution. Additionally, our methodology compares the output of several graph clustering algorithms in order to demonstrate the best-performing Graph Theoretical tools for studying galaxy evolution.

==> temp.tex <==
\bibliography{myrefs}
\begin{thebibliography}{}
\bibitem{AFPAInria}
V. Arsigny, P. Fillard, X. Pennec and N. Ayache: {\em Fast and Simple Computations on Tensors with Log-Euclidean Metrics}, INRIA Research Report, no. 5584, 2005.
\\

\bibitem{Barabasi2015} Barabási, A.-L., Network Science, Cambridge University Press in 2015.
\\

\textcolor{blue}{No need to give the titles in references in MN journal}\bibitem{Gephi} Bastian M., Heymann S., Jacomy M. : {\em  Gephi: an open source software for exploring and manipulating networks},  International AAAI Conference on Weblogs and Social Media (2009).
\\

\bibitem{BelNiy} M. Belkin, P. Niyogi : {\em Laplacian eigenmaps and spectral techniques for embedding and clustering}, Proceedings of Neural Information Processing Systems (NIPS), pp. 585-591 (2002).
\\

\bibitem{BeChrRe} C. Berg, JPR Christensen, P. Ressel : {\em Harmonic analysis on semigroups: theory of positive definite and related functions}, Springer (1984).
\\

\bibitem{Louvain} Vincent D Blondel, Jean-Loup Guillaume, Renaud Lambiotte, and Etienne Lefebvre:  {\em  Fast
unfolding of communities in large networks},  Journal of Statistical Mechanics: Theory and
Experiment, 2008(10), Oct 2008.
\\

\bibitem{BullmoreSpoon2009}  Bullmore, E., Sporns, O., Complex brain networks: {\em Graph theoretical analysis of structural and functional systems}, Nat Rev Neurosci, 10 (3), pp.186-98, Mar 2009.
\\

\bibitem{Brandetal} U. Brandes, D. Delling, M. Gaertler, R. Gorke, M. Hoefer, Z. Nikoloski, D. Wagner : {\em On modularity clustering}, IEEE Transactions on Knowledge and Data Engineering, vol. $20$, issue $2$ (2008).
\\

%\bibitem{Euler1736} Euler, Leonhard: {\em Solutio problematis ad geometriam situs pertinentis}, Comment. Acad. Sci. U. Petrop 8, 128–40  (1736).
%\\

 \bibitem{Fan} Fan R. K. Chung : {\em Spectral Graph Theory}, Regional Conference Series in Mathematics no. 92, 1997.
\\

\textcolor{blue}{This is a good example of giving references in MN journal}\bibitem{Farrah2009}  Farrah D., et al., ApJ, 700, 395, 2009.
\\

\bibitem{FasiTudi1} D. Fasino, F. Tudisco : {\em An Algebraic analysis of the graph modularity}, 
SIAM Journal on Matrix Analysis and Applications, vol. $35$ ($3$), pp 997 - 1018 (2014).
\\

\bibitem{FasiTudi2} D. Fasino, F. Tudisco : {\em Modularity bounds for clusters located by leading eigenvectors of the normalized modularity matrix}, Journal of Mathematical Inequalities, vol. $11$, Number $3$, pp. 701 - 714 (2017). 
\\

\bibitem{FasiTudi3} D. Fasino, F. Tudisco : {\em Generalized modularity matrices}, Linear Algebra and its Applications, vol. $502$, pp. 327 - 345 (2016).
\\

\bibitem{FasiTudi4} D. Fasino, F. Tudisco : {\em A modularity based spectral method for simultaneous community and anti-community detection}, Linear Algebra and its Applications, vol. $542$, pp. 605 - 623 (2018).
\\

\bibitem{GirvanNewman2002} M. Girvan and M. E. J. Newman: {\em   Community structure in social and biological networks}, 
Proceedings of the National Academy of Sciences, 99(12):7821-7826, 2002.
\\

\bibitem{GirvanNewman2004} M. E. J. Newman and M. Girvan:  {\em Finding and evaluating community structure in networks}, 
Phys. Rev. E, 69:026113, Feb 2004.
\\

\bibitem{Golan} J.S. Golan : {\em The Linear Algebra a beginning graduate student ought to know}, Springer 2012.
\\

\bibitem{ForceAtlas2} Jacomy M, Venturini T, Heymann S, Bastian M : {\em  ForceAtlas2, a Continuous Graph Layout Algorithm for Handy Network Visualization Designed for the Gephi Software}, PLoS ONE 9(6): e98679 (2014).
\\

\bibitem{JayHartley}
S. Jayasumana, R. Hartley, M. Salzmann, H. Li, M. Harandi : {\em Kernel methods on Riemannian manifolds with Gaussian RBF kernels}, IEEE Transactions on Pattern Analysis and Machine Intelligence, $37$ ($12$), pp. 2464 - 2477 (2015).
\\

\bibitem{Joll}
I. T. Jolliffe : {\em Principal Component Analysis, Second Edition}, Springer Series in Statistics, 2002.
\\

\bibitem{HofSchoSmo}
T. Hofmann, B. Sch\"{o}lkopf, A.J. Smola : {\em Kernel methods in Machine Learning}, The Annals of Statistics, 36(3): pp. 1171 - 1220 (2008).
\\

\bibitem{Hong2016} 
Hong S. et al: {\em   Discriminating topology in galaxy distributions using network analysis},  Monthly
Notices of the Royal Astronomical Society, 459(3):2690-2700 (2016).
\\

\bibitem{Hurley1}
P. D. Hurley, S. Oliver, D. Farrah, L. Wang and A. Efstathiou : 
{\em Principal component analysis and radiative transfer modelling of Spitzer Infrared Spectrograph spectra of ultraluminous infrared galaxies},  
Monthly Notices of the Royal Astronomical Society, 424(3):2069–2078, (2012). 
\\

\bibitem{Hurley2}
P. D. Hurley, S. Oliver, D. Farrah, V. Lebouteiller, H. W. W. Spoon :
{\em Learning the fundamental mid-infrared spectral components of galaxies with non-negative matrix factorization},  
Monthly Notices of the Royal Astronomical Society, 437(1):241-261, (2014).



\bibitem{Lian2007} J. Lian, Kshirasagar Naik, and G. B. Agnew: {\em   A framework for evaluating the performance
of cluster algorithms for hierarchical networks},  IEEE/ACM Transactions on Networking,
15:1478-1489, 2007.
\\

\bibitem{MaFu}
Y. Ma, Y.Fu : {\em Manifold Learning Theory and Applications}, CRC Press, 2011.
\\

\bibitem{MaPosHer}
L. V. D. Maaten, E. Postma and J. V. D. Herik: 
{\em Dimensionality Reduction: A Comparative Review},
 TiCC TR 2009-005, pp. 1-36, 2009.
\\

\bibitem{Novetal} 
J. Novembre, T. Johnson, K. Bryc, et al. : {\em Genes mirror geography within Europe}. Nature 456, 274 (2008).
\\

\bibitem{Newman2004} M. E. J. Newman:  {\em  Fast algorithm for detecting community structure in networks},  Phys. Rev.
E, 69:066133, Jun 2004.
\\

  \bibitem{Newman2006} M. E. J. Newman : {\em Finding community structure in networks using the eigenvectors of matrices}, Physical Review E 74, 036104, (2006).
\\

\bibitem{Newman2006b} M. E. J. Newman : {\em Modularity and community structure in networks}, Proceedings of the National Academy of Sciences of the United States of America, 103 (23), pp. 8577 - 8696 (2006).
\\


\bibitem{Radicchi} F. Radicchi, Cl. Castellano, F. Cecconi, V. Loreto, and D. Parisi: {\em  
Defining and identifying communities in networks},  Proceedings of the National Academy of Sciences, 101(9):2658-2663, 2004.
\\

\bibitem{ShCrist}
J. Shawe-Taylor, N. Cristianini :{\em Kernel Methods for Pattern Analysis}, Cambridge 2004.
\\

\bibitem{SchTR}
B. Sch\"{o}lkopf, A. Smola, K-R. M\"{u}ller : {\em Nonlinear Component Analysis as a Kernel Eigenvalue Problem}, Neural Computation, $10$ ($5$), pp. 1299 - 1319 (1998).
\\

\bibitem{Spoon2007} Spoon, H. W. W., Marshall, J. A., Houck, J. R., et al. 2007, ApJ, 654, L49
\\

\bibitem{StZw}
H. Strange, R. Zwiggelaar : {\em Open Problems in Spectral Dimensionality Reduction}, Springer Briefs in Computer Science, 2014.
\\


\bibitem{Leiden} V. Traag, L. Waltman, and N. J. van Eck:  {\em From louvain to leiden: guaranteeing
well-connected communities},  Scientic Reports, 9:5233, 03 2019.
\\


\bibitem{Ueda2003}, H., Takeuchi, T. T., and Itoh, M.: {\em  Graph-theoretical approach for comparison of observational galaxy distributions with cosmological N-body simulations}, Astrophysics and Astronomy, Feb 2003, Vol. 399, No. 1, pp. 1-7.
\\

\bibitem{VidMaSas}
R.Vidal, Y. Ma, S. S. Sastry : {\em Generalized Principal Component Analysis}, Interdisciplinary Applied Mathematics, vol. 40, Springer 2016.
\\

\bibitem{Xiaoetal}
L. Xiao, J. Sun, S. Boyd : {\em A duality view of spectral methods for dimensionality reduction} 
In: Proceedings of the $23$-rd International Conference on Machine Learning (ICML),
pp. 1041–1048 (2006).
\\

\bibitem{VanMieghem}
P. Van Mieghem : {\em Graph Spectra for Complex Networks}, Cambridge University Press, 2011.
\\

\bibitem{VanMieghemetal}
P. Van Mieghem, X. Ge, P. Schumm, S. Trajanovski, H. Wang : {\em Spectral graph analysis of modularity and assortativity}, Physical Review E $82$, $056113$ (2010). 

\bibitem{Wang}
Wang L., Farrah D.,Connolly B., Connolly N., LeBouteiller V., Oliver S., Spoon H.,2011, MNRAS, 411, 1809  

\textcolor{blue}{added some references here we may use}{\bf

\bibitem[Efstathiou(2006)]{efstathiou06} 
Efstathiou A.\ 2006, \mnras, 371, L70  \\

\bibitem[Efstathiou \& Rowan-Robinson(1995)]{efstathiour95} 
Efstathiou A., Rowan-Robinson M.\ 1995, \mnras, 273, 649 \\

\bibitem[Efstathiou \& Siebenmorgen(2009)]{efstathiou09} 
Efstathiou A., Siebenmorgen R.\ 2009, \aap, 502, 541 \\

\bibitem[Efstathiou et al.(1995)]{efstathiou95} 
Efstathiou A., Hough J.~H., Young S.\ 1995, \mnras, 277, 1134  \\

\bibitem[Efstathiou et al.(2000)]{efstathiou00} 
Efstathiou A., Rowan-Robinson M., Siebenmorgen R.\ 2000, \mnras, 313, 734  \\

\bibitem[Efstathiou et al.(2013)]{efstathiou13} 
Efstathiou A., Christopher N., Verma A., Siebenmorgen R.\ 2013, \mnras, 436, 1873  \\

\bibitem[Farrah et al.(2007)]{farrah07a}
Farrah D., Lacy M., Priddey R., Borys C., Afonso J.\ 2007, \apj, 662, 59  \\

\bibitem[Farrah et al.(2010)]{farrah10}
Farrah D. et al.\ 2010, \apj, 717, 868  \\

\bibitem[Farrah et al.(2012)]{farrah12}
Farrah D. et al.\ 2012, \apj, 745, 178  \\

\bibitem[Fischer et al.(2010)]{fisch10} 
Fischer, J., Sturm, E., Gonz{\'a}lez-Alfonso, E., et al.\ 2010, \aap, 518, L41  \\

\bibitem[Fritz et al.(2006)]{fritz06} 
Fritz, J., Franceschini, A., \& Hatziminaoglou, E.\ 2006, \mnras, 366, 767  \\

\bibitem[Gonz{\'a}lez-Alfonso et al.(2013)]{gonz13} 
Gonz{\'a}lez-Alfonso, E., Fischer, J., Bruderer, S., et al.\ 2013, \aap, 550, A25  \\


\bibitem[Herrero-Illana et al.(2017)]{herr17} 
Herrero-Illana, R., P{\'e}rez-Torres, M. {\'A}., Randriamanakoto, Z., et al.\ 2017, \mnras, 471, 1634. doi:10.1093/mnras/stx1672  \\

\bibitem[Houck et al.(2004)]{houck04} 
Houck, J.~R., Roellig, T.~L., van Cleve, J., et al.\ 2004, \apjs, 154, 18 \\

\bibitem[Klaas et al.(2001)]{klaas01} 
Klaas, U., Haas, M., M{\"u}ller, S.~A.~H., et al.\ 2001, \aap, 379, 823  \\

\bibitem[Kool et al.(2018)]{kool18} 
Kool, E.~C., Ryder, S., Kankare, E., et al.\ 2018, \mnras, 473, 5641. doi:10.1093/mnras/stx2463  \\

\bibitem[Mattila et al.(2018)]{matt18} 
Mattila, S., P{\'e}rez-Torres, M., Efstathiou, A., et al.\ 2018, Science, 361, 482. doi:10.1126/science.aao4669  \\

\bibitem[Nardini et al.(2009)]{nard09} 
Nardini, E., Risaliti, G., Salvati, M., et al.\ 2009, \mnras, 399, 1373 \\

\bibitem[Pitchford et al.(2019)]{pitch19} 
Pitchford, L.~K., Farrah, D., Alatalo, K., et al.\ 2019, \mnras, 487, 3130. doi:10.1093/mnras/stz1471 \\

\bibitem[Sanders \& Mirabel(1996)]{san96} Sanders, D.~B. \& Mirabel, I.~F.\ 1996, \araa, 34, 749  \\

\bibitem[Saunders et al.(2000)]{sau00} 
Saunders, W., Sutherland, W.~J., Maddox, S.~J., et al.\ 2000, \mnras, 317, 55  \\

\bibitem[Stalevski et al.(2016)]{stal16} 
Stalevski, M., Ricci, C., Ueda, Y., et al.\ 2016, \mnras, 458, 2288  \\

\bibitem[Sturm et al.(2011)]{sturm11} 
Sturm, E., Gonz{\'a}lez-Alfonso, E., Veilleux, S., et al.\ 2011, \apjl, 733, L16 \\

\bibitem[Veilleux et al.(2009)]{vei09} 
Veilleux, S., Rupke, D.~S.~N., Kim, D.-C., et al.\ 2009, \apjs, 182, 628

}

\end{thebibliography}

   \end{comment}

